Investigating the Indirect Object Identification circuit in Mamba

How well will current interpretability techniques generalize to future models? A relevant case study is Mamba, a recent recurrent architecture with scaling comparable to Transformers. We adapt pre-Mamba techniques to Mamba and partially reverse-engineer the circuit responsible for the Indirect Object Identification (IOI) task. Our techniques provide evidence that 1) Layer 39 is a key bottleneck, 2) Convolutions in layer 39 shift names one position forward, and 3) The name entities are stored linearly in Layer 39's SSM. Finally, we adapt an automatic circuit discovery tool, positional Edge Attribution Patching, to identify a Mamba IOI circuit. Our contributions provide initial evidence that circuit-based mechanistic interpretability tools work well for the Mamba architecture.

==> oldstuff.tex <==

\iffalse


 See appendix for a rough draft of this so far (but maybe that's too low level).

\subsection{IOI circuit in Transformers}



\subsection{Experiment Details of EAP-ACDC for MAMBA. }
\begin{itemize}
    \item Coarse to fine-grained circuit graph
    \item Gradient-descent like procedure to find subsets
    \item We separate by positions
\end{itemize}

To find this circuit, we:

Maybe modify -> do positional EAP and then prune convs
\begin{itemize}
    \item Used Edge Attribution Patching to estimate the contribution of each edge to a Normalized Logit Diff metric
    \item Sorted all edges by their contribution
    \item Used binary search to find the minimum number of edges needed to meet some target accuracy (85\% or 90\%)
    \item Pruned any edges that weren't along the path from embed to output
    \item Ran ACDC on the resulting graph (without positions)
    \item Ran ACDC on that graph (with positions)
\end{itemize}


Here is pruned graph obtained via Edge Attribution Patching

GRAPH HERE


Here is the first ACDC graph:

GRAPH HERE

And here is the final graph:

Our ACDC implementation has the following edges:

Edges between layers:

\begin{itemize}
    \item Embed $\mapsto$ Layer Input
    \item Layer Output $\mapsto$ Later Layer Input
    \item Layer Output $\mapsto$ Output Node
    \item Embed $\mapsto$ Output Node
\end{itemize}

Where Output Node is the residual stream after the final layer adds to it.

All of these edges use the standard edge patching: Consider an edge from layer i to layer j. We have

$$\text{patched\_layer\_input}_j = \text{layer\_input}_j - \text{layer\_output}_i + \text{corrupted\_layer\_output}_i$$

Where $\text{layer\_output}$ is computed during the same forward pass we are doing our patch, and $\text{corrupted\_layer\_output}_i$ is from a separate forward pass where we modify the token inputs.

We also have edges within each layer:
\begin{itemize}
    \item Layer Input $\mapsto$ Skip
    \item Skip $\mapsto$ Layer Output
    \item Layer Input $\mapsto$ Conv
    \item Conv $\mapsto$ SSM
    \item SSM $\mapsto$ Layer Output
\end{itemize}

(Skip $\mapsto$ Layer Output) and (SSM $\mapsto$ Layer Output) are dummy edges that are always present, just used to represent the flow of information/ensure the graph is connected.

(Layer Input $\mapsto$ Skip) is a (non-edge) patch that overwrites the value with the value from a corrupted run.

(Layer Input $\mapsto$ Conv) has an edge for each conv filter, where a patch for filter i overwrites that filter's inputs with corrupted values. This was tricky to implement correctly, we recommend looking at the code for more information.

(Conv $\mapsto$ SSM) is a (non-edge) patch that overwrites the hidden state with the corrupted hidden state.

We would like to get a more fine-grained view of which tokens are being used where, but by default ACDC doesn't allow that. To address this, during the second ACDC pass, we duplicate all edges num\_tokens times, and give them a token\_position parameter. This only applies the patch at that token position, instead of all token positions.

We used ACDC thresh of 0.001.

\section{Circuit discovery experiments}

\subsection{Adding one layer at a time}

Experiments that start will all layers patched, then unpatch one layer at a time until minimal graph is found

\subsection{Mamba is robust to layer removal}

Completely removing layers, one at a time, and plotting performance on task.

Plot that has remove one layer at a time, shows loss slowly decrease

Plot that shows effect of removing each layer
- Evidence that 39 is bottleneck
- Evidence that there is a shared representation space.

What if we take the linear representation of names and put that     into the residual stream some layers before 39?
- insert in final position, does that overwrite? Like take average of what 39 outputs to residual stream and stick that earlier?
- Or what 39 takes in

\section{39 Conv attend to previous token}
    
Patching that shows conv on layer 39 fetches previous token. Figured that out by patching to a conv filter. 39 negative 1 lines up if you do that

\section{Hidden state cosine sim lens}

Describe the lens, say that because it's a saliency map it's a lil sus, show fragility to choice of names

\section{Reading and writing names from layer 39}
as
Explain the averaging thing.

Linear probes here didn't work, likely because the information is already everywehr

\subsection{Substitution}

5x5 substitution graph

\subsection{What are the name representations?}

PCA of repesentations, top components is templates, so don't include templates

What is PCA now?

Umap?

\subsection{Specific pairs of names that are exceptions}

\section{Future work}

Feature circuits




\section{Appendix stuff}

In the \emph{circuit} perspective, neural networks are broken up into nodes (layers, heads, etc.), where the edges between those nodes represent information flowing through the network. By default, this graph is too large to analyze (Mamba 370m has 49 layers so at a minimum this graph has ~$49^2$ edges), so we want to prune edges that are unimportant for accomplishing the task we are interested in.

There are two key tasks here: 1) what does it mean to prune an edge, and 2) which edges should be pruned.

\subsection{What does it mean to prune an edge}

Consider an edge that goes from a node representing layer 4 to a node representing layer 6. Recall that each layer adds to the residual stream, which is then the input for later layers.

If we want to prune this edge, we have a few options:
\begin{itemize}
\item Zero ablation: Zero out the contribution of layer 4 to the residual stream
\item Mean ablation: Compute the mean of 4's output over many data points, and use that as 4's output
\item Noise ablation: Compute random noise for 4's output
\end{itemize}

Unfortunately, these three options all result in activation values that are "unnatural": outside the typical distribution we might see on the task.

A better alternative is called activation patching (also known as interchange interventions and causal tracing):
\begin{enumerate}
    \item Modify the prompt to create a "corrupted" prompt (for example, by replacing a name with a randomly chosen different name)
    \item Run a forward pass on the corrupted outputs and record the activations
    \item "Patch" the activations into our original stream
\end{enumerate}

In our example, we would replace layer 4's output with layer 4's output from the corrupted run. Because each layer adds to the residual stream, we represent patching our $4 \mapsto 6$ edge via

$\text{patched layer input}_6 = \text{layer input}_6 - \text{layer output}_4 + \text{corrupted layer output}_4$

Where $\text{layer output}_4$ is computed during the same forward pass as $\text{layer input}_6$ and $\text{patched layer input}_6$, and $\text{corrupted layer output}_4$ is stored values from a sepearte forward pass using the corrupted prompt.

There are many choices for nodes. A very high level choice of nodes could be:
\begin{itemize}
    \item an "input" node that corresponds to the token embedding
    \item a node for every layer
    \item an "output" node that corresponds to the residual stream after the final layer has added to it
\end{itemize}

\subsection{Which edges should be pruned?}

The simplest algorithm is to:
\begin{enumerate}
    \item Topologically sort edges
    \item $\text{edges patching} = \text{[]}$
    \item For each edge, starting from the highest (the ones connected to the sink):
    \begin{enumerate}
        \item Baseline accuracy = patch all edges in edges patching
        \item Edge accuracy = patch all edges in edges patching \emph{and} this edge
        \item Accuracy diff = Edge accuracy - Baseline accuracy
        \item If this diff isn't too large, add this edge to edges patching
    \end{enumerate}
    \item Prune any edges that don't have a path from source to sink
\end{enumerate}

This is (almost) the ACDC algorithm. The motivation for starting from the sink and working backwards is that earlier edges may affect the outputs of later edges.

There are two issues with this algorithm:
\begin{enumerate}
    \item Accuracy isn't a great metric, there are types of circuits that it misses
    \item This takes a forward pass for every edge. If we have ~$49^2$ edges this can take a long time.   
\end{enumerate}

\subsection{Accuracy isn't a great metric}

What metric is best is still an open question and seems to be task specific. However, for indirect object identification, normalized logit diff is the preferred metric.

Consider the case where we have the "correct" answer A, and the incorrect answer B. B is also the correct answer for our "corrupted" prompt. Normalized logit diff does:

\begin{enumerate}
    \item $\text{min\_diff} = \text{A\_logit\_corrupted} - \text{B\_logit\_corrupted}$
    \item $\text{max\_diff} = \text{A\_logit\_unpatched} - \text{B\_logit\_unpatched}$
    \item $\text{possible\_range} = (\text{max\_diff}-\text{min\_diff})$
    \item $\text{possible\_range[possible\_range == 0]} = 1 \text{\# prevent divide by zero}$
    \item $\text{logit\_diff} = \text{A\_logits\_patched} - \text{B\_logits\_patched}$
    \item $\text{normalized\_logit\_diff} = (\text{logit\_diff}-\text{min\_diff})/\text{possible\_range}$
\end{enumerate}

where

\begin{itemize}
    \item unpatched is a forward pass without our intervention (the baseline forward pass)
    \item corrupted is a forward pass without our intervention, where the prompt is modified to make B the correct answer
    \item patched is a forward pass that patches edges (as described above)
\end{itemize}

This gives us a 1 when the model acts like the unpatched forward pass, and 0 when the model acts like the corrupted forward pass.

In general, we can just talk about a "Metric" that returns a scalar value to be maximized. KL-Divergence and unnormalized logit diff are also of interest.

\subsection{ACDC is too slow}

Instead of patching one edge at a time, edge attribution patching uses two forward passes and one backward pass to simultaneously estimate the contribution all edges has to our metric.

Consider the edge from layer i -> layer j. Recall from above, we apply that intervention via

$$\text{patched\_layer\_input}_j = \text{layer\_input}_j - \text{layer\_output}_i + \text{corrupted\_layer\_output}_i$$

Call 

$$\text{diff}_i = - \text{layer output}_i + \text{corrupted layer output}_i$$

So we can write

$$\text{patched\_layer\_input}_j = \text{layer\_input}_j + diff_i$$

Now, write our metric as

$$\text{Metric}(\text{input\_tokens}, \text{diff})$$

TODO

This lets us approximate the attribution of our (i,j) edge as

$$\text{diff}_i*\nabla(\text{layer\_input}_j)$$

Where $\nabla(\text{layer\_input}_j)$ is computed via a backwards hook on $layer\_input_j$.




make hypotheses about what they are processing and try intervening in those ways



\section{Contributions}
\begin{itemize}
    \item Brief/legible explanation of Mamba. Short version and refer people to Ophiology.
    \item Cosine similarity per step
    \item Abstraction
    \item Layer removal: a different version of patching,   essentially zero-ablating layers. It's best as a small note.
    \item Conv 39 (patching and ACDC)
    \item Reading and writing names
    \item Linear probes too powerful at names
    \item PCA on name averages (used to read and write), but not with template (because templates dominated)
    \item Batched ACDC (just mention as a paragraph) and batched patching, not as relevant for EAP (tho I did batch it)
    \item we can just link Mamba lens and InputDependentHookPoint, sentence and a link 
    \item Direct Logit Attribution? (wasn't too helpful, maybe just mention)
    \item Logit lens? (they already did that so don't bother)
\end{itemize}


Todos? For later paper
\begin{itemize}
    \item Fill out the graph of 5x5? Might be too much
\end{itemize}

%State space models are based around mapping an $E$-dimensional space to a $N$-dimensional space, then back to an $E$ dimensional space:

%$$\stackrel{[N]}{\dot{h}(t)} = \stackrel{[N,N]}{A}\stackrel{[N]}{h(t)} + \stackrel{[N,E]}{B}\stackrel{[E]}{x(t)}$$
%$$\stackrel{[E]}{y(t)} = \stackrel{[E,N]}{C}\stackrel{[N]}{h(t)} + \stackrel{[E,E]} D\stackrel{[E]} x(t)$$

%$\dot{h}(t)$ is the derivative of $h(t)$ with respect to time, t. Writing this as a recurrence gives us

%$$\stackrel{[N]}{h_{t}} = \stackrel{[N,N]}{\overline{A}}\stackrel{[N]}{h_{t-1}} + \stackrel{[N,E]}{\overline{B}}\stackrel{[E]}{x_{t}}$$
%$$\stackrel{[E]}{y_t} = \stackrel{[E,N]}{C}\stackrel{[N]}{h_t} + \stackrel{[E,E]} D\stackrel{[E]} x_t$$

%where $\overline{A}$ and $\overline{B}$ are our *discretization matrices*. Mamba uses a mix of zero-order hold (ZOH) and Euler Method to give discretization matrices of

%$$\overline{A} = \exp(\Delta A)$$
%$$\overline{B} = \Delta B$$


    
Doing this helps us understand the direct and indirect effects of each layer.






Papers to cite:
- Emergent Abilities of Large Language Models Wei 2022
-- People are interested in studying what capabilities large language models have, mech interp helps us do that
- Kaplan 2020
-- Scaling laws are high level but we don't have low level
- Alishahi 2019 Fong 2017 Buhrmester 2021
-- LLMs are black boxes
- Lipton 2016
--  LLMs are not black boxes
- Olah 2022
-- What mech interp is trying to do (turn black boxes into algorithms we can understand)
- Geiger 2021
-- Computational graph perspective
- Wang 2023
-- Circuits are subgraphs of that computational graph
- Rauker 2022
-- Initial manual extraction of circuits
- Conmy 2023
-- ACDC
- Cao 2021
-- Subnetwork Probing
- Michel 2019
-- Head Importance Score for Pruning
- Hanna 2023
-- Greater than task
- Heimersheim 2023
-- Docstring
- Goldowsky-Dill 2023
-- Induction
- Wang 2023
-- IOI Task
- Nanda 2023 Chughtai, Chan, and Nanda 2023
-- Fully reverse enginer algorithm for toy model
- Elhage 2021
-- Residual stream is additive so you can patch via subtract and add
- Pearl 2009
-- Causal inference stuff, it's Pearl duh
- Vig 2020
-- ??? Something about direct vs mediated interaction, indirect effects, etc.
- Olsson 2022 Cammarata 2021
-- Zero ablation
- Wang 2023 
-- Mean ablation
- Geiger 2021
-- Interchange interventions/resample ablation
- Chan 2022
-- Zero and mean ablation are unnatural
- Hanna 2023 Heimersheim 2023 Wang 2023
-- ppl that use interchange interventions
- Olah 2017 Elhage 2022
-- mech interp is about trying to understand features learned by models
- Elhage 2021
-- mech interp is about mathematical frameworks for understanding architectures ?? (is this the reverse engineering modular stuff work?)
- Nanda 2023 Cammarata 2021 Chughtai 2023 Wang 2023
-- mech interp is about circuits
- Fu 2023
-- mech interp used to inspire better architectures
- Bills 2023
-- use llms to label neurons
- LeCun 2989
-- prune neurons/weights
- Wang 2020 Kurtic 2022
-- prune to to make network more sparse (usually to compress networks or to get faster inference)
- Hassibi 1992
-- said that if we prune networks they'll be more interpretable
- Grover 2022
-- rip the pruning interpretability dreams
- Louizos 2018 Wang 202 Cao 2021
-- Balance model performance and network sparsity to learn mask from data
- Frantar 2023
-- learnable masks don't change weights of model after pruning
- Michel 2019
-- use magnitude of gradients to pick which nodes to prune
- Sanh 2020
-- removes parameters that have "a high velocity to a low magnitude"?? (idk what that means)
- Zhu 2023
-- Pruning and other compression techniques
- Pearl 2009 Feder 2021 Geiger 2021 Wu 2022 Kaddour 2022
-- causal explanations of model outputs
- Vig 2020
-- indirect effects vs direct effects in LLMs something about proxies??
- Goldowsky-Dill 2023
-- Path patching
- Wu 2023
-- Causal Testing to see whether nns implement a given algorithm
- Veit 2016
-- Explain training dynamics via paths in the computational graph
- Geva 2021
-- MLP are associative memory
- Elhage 2021
-- Residual is sum of all different paths
- Bau 2020 Meng 2022
-- Look at subgraphs to edit behavior
- Chan 2022
-- USe subgraphs to test hypotheses

\fi

